Explicitly Modeling Syntax in Language Models with Incremental Parsing and a Dynamic Oracle

Syntax is fundamental to our thinking about language. Failing to capture the structure of input language could lead to generalization problems and over-parametrization. In the present work, we propose a new syntax-aware language model: Syntactic Ordered Memory (SOM). The model explicitly models the structure with an incremental parser and maintains the conditional probability setting of a standard language model (left-to-right). To train the incremental parser and avoid exposure bias, we also propose a novel dynamic oracle, so that SOM is more robust to wrong parsing decisions. Experiments show that SOM can achieve strong results in language modeling, incremental parsing and syntactic generalization tests, while using fewer parameters than other models.

==> intro_old.tex <==
\section{Introduction}

Natural language is the result of the interplay between several linguistic phenomena such as syntax, semantics and pragmatics.
Current language models confound these phenomena, making it hard to assess their linguistic ability.
Several recent works systematically study the linguistic abilities of modern language models, especially syntax  \cite{linzen2016assessing,marvin2018targeted,gulordava2018colorless}.
Their main findings are that 1) most language models are good at capturing frequent syntactic structures but do not generalize well to those in the long tail and 2) although some excel at having low perplexity scores, this is less due to their syntactic ability but more to their capturing collocations (frequently co-occurring words).
More recently, \citet{hu2020systematic} show that RNNs are bad at syntactic generalization, whereas models that have an explicit notion of syntax fare well but at the cost of language modeling (higher perplexity).
On the other hand, transformer-based models achieve strong performance when trained with large datasets, but are worse than random when trained on a small dataset.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/high_level_idea.PNG}
    \caption{The mechanism of SOM.
    ``\textit{Context}'' is a distributed representation of previous sentences. 
    It could also represents the source sentence in a sequence to sequence task.
    It incrementally build subtrees given the input sentences. 
    A RNN will takes the context representation and the representations of subtrees in the current sentence to predict next token.
    }
    \vspace{-0.5cm}
    \label{fig:high_level}
\end{figure}

In this work, we propose a new model, Syntactic Ordered Memory (SOM), that models explicit syntax and can also achieve strong language modeling and syntactic generalization performance on both small and large corpora.
Inspired by psycholinguistic evidence \cite{marslen1973linguistic,altmann1988interaction,tanenhaus1995integration} that humans language processing is incremental, SOM incrementally models syntactic structure, then use the structure as computation graph to predict the next token.
% Inspired by psycholinguistic evidence that humans language processing is incremental, we make the syntactic parser component of the language model incremental .
In other words, the parser makes a syntactic decision that influences the language model predictions at each time step.
The parse is represented as a distributed Ordered Memory \cite{shen2019ordered}, %the order dictated by the syntactic structure,
and the language model predicts a word conditioned on this ordered memory. 
Fig.\ref{fig:high_level} shows the mechanism of SOM.

We also investigate if disentangling syntax from a language model improves generalization.
Our motivation comes from the observation that syntax is autonomous from other linguistic phenomena, i.e., one can form syntactically valid sentences even if they are meaningless, e.g., the now infamous sentence from \citet{chomsky1956syntactic}: \textit{Colorless green ideas sleep furiously}.
We make a language model competent at syntax through supervision from annotated data.

We compare our model with existing proposals of integrating syntax into language models.
RNNGs \citep{dyer2016recurrent}, Ordered Neurons \citep{shen2018ordered} and Ordered Memory \citep{shen2019ordered}, in particular are closely related.
RNNGs are generative models of language which define a joint distribution on syntactic structures and sequence of words.
%Ordered Neurons models syntactic structures as a latent variable, and try to marginalize over the latent structure to achieve better performance on language modeling.
Ordered Neurons attempt to model the hierarchical structure of language by defining an ordering to the hidden states and the gates that impose that structure.
Ordered Memory functions like a stacked based incremental parser with a one-step look-ahead.
Consequently, it maintains a latent tree structure for the sequence.
%But it also models syntactic structures as a latent variable. 
Based on the Ordered Memory, we propose the SOM which models a joint distribution like RNNG. 
But there are several important differences from previous models:
\begin{itemize}
    \item Instead of using teacher forcing to train the incremental syntactic parser, we borrow techniques from imitation learning with our Adaptive Structural Loss.
    %The new loss function does not carry forward penalties the model makes early on in the parse.
    The new loss function generates structure labels on the fly, conditioning on the gold tree and faults made by the model earlier. This makes the model more robust at test time, given that it is directly trained to cope with its own parsing decisions.
    \item We introduce a dedicated prediction network to predict the next token. While the Ordered Memory use a one-step look-ahead parser to predict the structure for current input token, the prediction network is equipped with a zero-step look-ahead parser to predict the structure for next token.
    \item We provide a way to implement the autonomy of syntax in SOM, which uses a disentangled representation to model syntactic structure.
\end{itemize}
In terms of performance, our model achieves strong performance on language modeling, syntactic generalization, and incremental parsing tasks. 
We also find consistent evidence that our disentangled model achieve better generalization in the out-of-domain generalization.

% Story:
% RNNs confound many things -- syntax, semantics, pragmatics etc.
% Syntax provides scafolding
% LM builds on the scafold
% Word is generated based on the syntax
% If structure is committed until the last word, there is no way to correct
% Commit until the last word -- mimic lookahead for one word
% Language model based on the sytactic structure and the last word. 
% Disentangling -- lower number of parameters (since syntax can be modeled with fewer parameters, and conditioned on syntax becomes easy)
% Better syntactic generalization (losely factoring out syntax)

% Commenting to shift to a later place.
%Due to the incremental nature of our parser, depending on the word predicted, our syntactic parse may change.
%In order to alleviate this problem partially, we commit to a parse only up to the last but one word, and for the last word, we have multiple parse possibilities from which one will be favored only after the language model commits to a word.
% \siva{can we have a nice figure on the first page that gives a high level idea}
% \alex{we can cite some works on surprisal,  cite maybe the case of garden path sentences.}
% High-level interaction between syntax and language model is shown in Figure~\ref{fig:simple-figure}.
% To account for this, we commit to a structure in only after looking at the word, i.e., one lookahead operation.

%Still, syntax is a prerequisite for forming meaningful sentences, providing scaffolding for sentences upon which words stand to form meaningful sentences.
%This scaffolding does not change across corpora, so learning the right syntactic structure may afford the same benefits as having the right inductive priors in other settings.
%For convolutional nets, it has allowed models to learn faster and from less data.
%\alex{Syntax doesn't change across corpora, learn faster, from less data, etc.}
%\siva{Excellent point! This has to be in the introduction to highlight why syntax helps generalization}
%\yikang{I don't know if we have enough proof for this point}
% Therefore, any good language model should be competent at syntax.
%Since syntax is well studied and has abundant resources, we make a language model competent at syntax through supervision from annotated data.
% We do so by providing it external supervision -- syntax as defined by linguists.



% Existing transition-based parsers are lookahead parsers -- without lookahead their performance drops significantly
% Incremental parsers either use a beam search or recorrect thier interpretation at every time stamp. Strictly predictive parsers are limited (with simple syntax).
% Point on training both in the same objective is hard because lexical actions, which advance the analysis onwards to successive words, are assigned such  probabilities compared to structural actions which do not advance to the next word (Stern et al. 2017) quoted in Hale et al. Requires a discriminative parser to sample trees at inference time.
% Marvin and Linzen good example of jointly training syntax and LM. Equal importance to both syntax and LM.

% \siva{Our model is also a joint model right? I am having hard time highlighting the differences. Is there a way to define formally the difference between a disentangled model and a joint model. Probably we need less number of parameters. Also, it is possible to distinguish disentagling from multi-tasking somewhere (may be in the related work).}
% \alex{few ideas: RNNGs (a) don't have one-step look-ahead while generating; (b) are trained by teacher forcing (we found this to perform worse that s why we have imitation-learning-like loss in 3.3); (c) worse performance on language modeling}
% \todo{shawn: how's this?}
% In terms of performance, we find that our model generalizes well both on syntactic tasks and language modeling (lower perplexity).

% Comparing to Ordered Memory, the adaptive structural loss provide a supervised and controllable way to learn the complex syntactic structure of natural language. 
% We also introduced the prediction network to allow the model perform better on language modeling.
% And disentangling the syntactic 

% Our main difference is our model requires fewer parameters due to the disentangled nature --- the syntactic component models syntax, and the language model 
% This makes inference on the language modeling slow (either to get a MAP estimate or the full parse).
% TODO.
% Whereas in our case, the language model inference is fast due to the disentangled nature --- the language model just relies on the parse.



% \siva{I think we also need a small paragraph describing the model architecture comparing it to ordered memory, and the new components.}
% \yikang{I will do it.}
% Our contributions are as follows:


% RNNGs are generative models of language which define a joint distribution on syntactic structures and sequence of words.
% This makes inference on either syntax or language modeling alone intractable, and one has to resort\alex{Mmmh, I have doubts that this is true.} to approximate estimations.
% Shawn:
% Inference is not actually hard (sentence -> parse), that's the q(y|x) model.
% To get the argmax of q(y|x) I believe you can do some kind of beam search, it's similar for our model except that ours even during training we've taken argmax greedily
% The "hard" thing is approximating p(x), which is the part that requires importance sampling.
% Because we have chosen to go with argmax in the slot selection, and the next time step slot selection is not conditioned on the stochastic decision of the previous step.
% Seems to me the novel stuff we have over the RNNG are 1) disentangling the syntax/semantics and 2) relative encoding of stack positions


% \begin{itemize}
% \item syntax + semantics is good for robustness , adaptation , low-data etc.
% \item Modeling both syntax and semantics well in a single model has seemed difficult. Models that are good at syntax usually show high perplexity. Good language models usually don t have explicit syntax representation. (mention to what extent syntax seem to be captured implicitly in current models)

% \item Most syntax-semantics model recur to discrete decisions to model the structure (~i.e. parametrize variants of shift-reduce parser (SPINN / RNNG / RRNet)) which makes them hard to train in an unsupervised way
% \yikang{We also make discrete decisions in this work, and we can't train it in an unsupervised way for now.}
% \item Some hypothesis because we fare well are: i) disentangling of syntax and semantics in the same model; ii) parsing-as-attention, we can train our model without recurring to high variance RL techniques which have been shown to be difficult to train in this setting; iii) relative prediction loss which is related to imitation learning.
% \end{itemize}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.75\linewidth]{figures/disentanglement.PNG}
%     \caption{The schema of disentangling syntax from language model. 
%     The language model output depends on both semantic and syntactic input, and it can backpropagate into both input.
%     While the structure also depends on both input, it can only backpropagate into the syntactic input.
%     }
%     \label{fig:disentanglement}
% \end{figure}
% Siva background research
% Excerpts from other papers 


% Predictive Incremental Parsing Helps Language Modeling -- very relevant
% Conditioning N-gram models, MaxEnt models or RNN-LMs on parser predictions yields perplexity reductions of about 6 %. Our method (a) retains online decoding capabilities and (b) incurs relatively little computational overhead which sets it apart from previous approaches that use syntax for language modeling.
% We use the prediction about the upcoming word types for language modeling, following the intuition that e. g. a verb might be more likely when the parser predicts that a verb is missing to complete the sentence.

% URNNG: Recurrent neural network grammars (RNNGs) (Dyer et al., 2016) model sentences by first generating a nested, hierarchical syntactic structure which is used to construct a context representation to be conditioned upon for upcoming words. Supervised RNNGs have been shown to outperform standard sequential language models, achieve excellent results on parsing

% Hale et al: with a parsing procedure that uses this grammar to manage a collection of syntactic derivations as it advances from one word to the next


% We want 
%  Good generative model
%   Good by what standards? Perplexity and syntactic generalisation
%    What better way than to train explicitly on syntactic information and language modelling

% What exists that already does this?
%  RNNG - also uses a stack parser and predicting the next word using the stack
%         but e.g. perplexity scores weren't great, not really incremental because of
%         autoregressive latent structure
%  RNNs - can learn _some_ common syntactic structures but fail when it comes to longer-term structures (Guldorova; ON; ...)
% Transformer-family - Hu showed that GPT-2 is dependent on scale of dataset.


